A Hybrid 3DCNN and 3DC-LSTM based model for 4D Spatio-temporal fMRI data: An ABIDE Autism Classification study

Functional Magnetic Resonance Imaging (fMRI) captures the temporal dynamics of neural activity as a function of spatial location in the brain. Thus, fMRI scans are represented as 4-Dimensional (3-space + 1-time) tensors. And it is widely believed that the spatio-temporal patterns in fMRI manifests as behaviour and clinical symptoms. Because of the high dimensionality ($\sim$ 1 Million) of fMRI, and the added constraints of limited cardinality of data sets, extracting such patterns are challenging. A standard approach to overcome these hurdles is to reduce the dimensionality of the data by either summarizing activation over time or space at the expense of possible loss of useful information. Here, we introduce an end-to-end algorithm capable of extracting spatiotemporal features from the full 4-D data using 3-D CNNs and 3-D Convolutional LSTMs. We evaluate our proposed model on the publicly available ABIDE dataset to demonstrate the capability of our model to classify Autism Spectrum Disorder (ASD) from resting-state fMRI data. Our results show that the proposed model achieves state of the art results on single sites with F1-scores of 0.78 and 0.7 on NYU and UM sites, respectively.

==> results_NYU.tex <==
\begin{center}
\begin{table}[]
\centering
\caption{Accuracy and F1 scores of Models on NYU data}
\label{tab:results}
\begin{tabular}{c|c|c}
\textbf{Model} & \textbf{Accuracy} & \textbf{F1 score} \\ \hline
SVM            &                   &                   \\
Heinsfeld      &                   &                   \\
1DConv         &                   &                   \\    
3DCNN\_1Dconv  &     57            &      58          \\
3DConvLSTM     &                   &                   \\ \hline
\end{tabular}
\end{table}
\end{center}

==> results_UM.tex <==
\begin{center}
\begin{table}[]
\centering
\caption{Accuracy and F1 scores of Models on UM data}
\label{tab:resultsUM}
\begin{tabular}{c|c|c}
\textbf{Model} & \textbf{Accuracy} & \textbf{F1 score} \\ \hline
SVM            &                   &                   \\
Heinsfeld      &                   &                   \\
1DConv         &                   &                   \\    
3DCNN\_1Dconv  &                   &                   \\
3DConvLSTM     &                   &                   \\ \hline
\end{tabular}
\end{table}
\end{center}
